Enablers and Impediments for Collaborative Research in Software Testing: An Empirical Exploration

When it comes to industrial organizations, current collaboration efforts in software engineering research are very often kept in-house, depriving these organizations off the skills necessary to build independent collaborative research. The current trend, towards empirical software engineering research, requires certain standards to be established which would guide these collaborative efforts in creating a strong partnership that promotes independent, evidence-based, software engineering research. This paper examines key enabling factors for an efficient and effective industry-academia collaboration in the software testing domain. A major finding of the research was that while technology is a strong enabler to better collaboration, it must be complemented with industrial openness to disclose research results and the use of a dedicated tooling platform. We use as an example an automated test generation approach that has been developed in the last two years collaboratively with Bombardier Transportation AB in Sweden.

==> sections/related.tex <==
\indent Several methods have been developed for the formal analysis
and verification of {\east} models. Nallet et al. \cite{5232001}
describe the use of UML MARTE profile \cite{ANDRE-2007-204484}
for {\east} with the purpose of performing timing analysis. In addition, Feng et al. \cite{5588261} propose
a translation of {\east} activity diagrams  into the input language of the SPIN model checker for formal verification. More recently, Qureshi
et al. \cite{qureshi} describe a model-to-model transformation from {\east} to timed automata
towards formal verification based on timing constraints using {\uppaal}. Related to this work, in the context of model-driven development, Biehl et al. \cite{biehl2010modular} are reporting their experiences from applying two model transformations in practice: (i) from Simulink to EAST-ADL and (ii) from EAST-ADL to HiP-HOPS for reliability analysis.
